Up or Down? Adaptive Rounding for Post-Training Quantization

When quantizing neural networks, assigning each floating-point weight to its nearest fixed-point value is the predominant approach. We find that, perhaps surprisingly, this is not the best we can do. In this paper, we propose AdaRound, a better weight-rounding mechanism for post-training quantization that adapts to the data and the task loss. AdaRound is fast, does not require fine-tuning of the network, and only uses a small amount of unlabelled data. We start by theoretically analyzing the rounding problem for a pre-trained neural network. By approximating the task loss with a Taylor series expansion, the rounding task is posed as a quadratic unconstrained binary optimization problem. We simplify this to a layer-wise local loss and propose to optimize this loss with a soft relaxation. AdaRound not only outperforms rounding-to-nearest by a significant margin but also establishes a new state-of-the-art for post-training quantization on several networks and tasks. Without fine-tuning, we can quantize the weights of Resnet18 and Resnet50 to 4 bits while staying within an accuracy loss of 1%.

==> tables/_old_exp_05_different_data.tex <==
\begin{table}[t]
    \centering
    \begin{tabular}{ l r r r }
        \toprule
         Data set          & 256 imgs  & 512 imgs & 1024 imgs \\\midrule
         ImageNet (train)            &  68.17$\pm$0.07   & 68.34$\pm$0.08 & 68.42$\pm$0.07 \\
         Pascal VOC    & XXX\%   &  XXX\% \\
         MS Coco    & XXX\%   &  XXX\% \\
         \bottomrule 
    \end{tabular}
    \caption{Top1 ImageNet validation results for Resnet18 optimized with different amount of images from various datasets. The weights of all layers are quantized with 4 bit symmetric quantization using our proposed LTR approach.}
    \label{tbl:exp5_data_sets}
\end{table}

% Run command   -- Note: results with linear annealing!!!
% Num samples and DS			
% Base options: ['validate_quantized', '--cuda', '--images-dir', '/local/mnt/workspace/imagenet/', '--architecture', 'resnet18_quantized', '--qmethod', 'symmetric', '--freeze-bn', '--n-bits', '4', '--no-act-quant', '--batch-size', '64', '--learn-to-round', 'all', '--ltr-weight', '0.0001', '--ltr-mode', 'learned_hard_sigmoid', '--ltr-asym', '--ltr-init', 'mse']			
			
% Final results (5 runs):	ImageNet		
% Opt1 \ Opt2 	 ['--ltr-iters', '10000']	 ['--ltr-dataset', 'mscoco']  	  ['--ltr-dataset', 'pascalvoc']
% ['--num-ltr-samples', '256'] 	 68.17 (+-0.07) 		
% ['--num-ltr-samples', '512'] 	 68.34 (+-0.08) 	 68.16 (+-0.08) 	 68.21 (+-0.09) 
% ['--num-ltr-samples', '1024'] 	 68.42 (+-0.07) 	 68.27 (+-0.08) 	 68.28 (+-0.08)
% ['--num-ltr-samples', '1536'] 	 68.49 (+-0.12) 		
% ['--num-ltr-samples', '2048'] 	 68.50 (+-0.05) 	 68.36 (+-0.06) 	 68.36 (+-0.08) 


==> tables/table_template.tex <==
%DUMMY table
\begin{table}[t]
    \centering
    \begin{tabular}{ l r r }
        \toprule
         HEADER          & FP32      & INT8 \\\midrule
         Row 1 & XXX\%   &  XXX\% \\
         Row 2 & XXX\%   &  XXX\% \\
         \bottomrule \\ 
    \end{tabular}
    \caption{TODO}
    \label{tbl:TODO}
\end{table}

